Pluggable AOP: Designing Aspect Mechanisms for Third-party Composition

Studies of Aspect-Oriented Programming (AOP) usually focus on a language in which a specific aspect extension is integrated with a base language. Languages specified in this manner have a fixed, non-extensible AOP functionality. In this paper we consider the more general case of integrating a base language with a set of domain specific third-party aspect extensions for that language. We present a general mixin-based method for implementing aspect extensions in such a way that multiple, independently developed, dynamic aspect extensions can be subject to third-party composition and work collaboratively.

==> aop1code.tex <==
aop1 {
	around: and(pexecution(Improve) args(an,x,epsilon)) {$\label{aop1:around1:start}$
		/(+(an,/(x,an)),2)
	}$\label{aop1:around1:end}$
	around: and(pexecution(IsPreciseEnough?) args(root,x)) {$\label{aop1:around2:start}$
		lt? (call Abs(-(x,call Square(root))),call Precision(x))
	}$\label{aop1:around2:end}$
	around : pcall(Precision) {$\label{aop1:around3:start}$
		/(proceed,1000)
	}
}$\label{aop1:around3:end}$


==> aop2code.tex <==
aop2 { guard_cflow SQRT resume_with call Precision(1) }


==> basecode.tex <==
program {
	procedure SQRT(radicand) {
		call SqrtIter(0,radicand,call Precision(radicand))
	}
	procedure SqrtIter(approximation,radicand,precision) {
		let
			bid = call Improve(approximation,radicand,precision)
		in
			if call IsPreciseEnough?(bid,radicand) 
			then bid
			else call SqrtIter(bid,radicand,precision)
	}
	procedure Improve(approximation,radicand,precision) {
		+(approximation,precision)
	}
	procedure Precision(x) {1}
	procedure IsPreciseEnough?(root,square) {
		lt?(square,call Square(root)) 
	}
	procedure Square(x) {*(x,x)}
	procedure Abs(x) {if lt?(x,0) then -(0,x) else x}
	procedure main() {call SQRT(5)}
}

